WeakSTIL: Weak whole-slide image level stromal tumor infiltrating lymphocyte scores are all you need

We present WeakSTIL, an interpretable two-stage weak label deep learning pipeline for scoring the percentage of stromal tumor infiltrating lymphocytes (sTIL%) in H&E-stained whole-slide images (WSIs) of breast cancer tissue. The sTIL% score is a prognostic and predictive biomarker for many solid tumor types. However, due to the high labeling efforts and high intra- and interobserver variability within and between expert annotators, this biomarker is currently not used in routine clinical decision making. WeakSTIL compresses tiles of a WSI using a feature extractor pre-trained with self-supervised learning on unlabeled histopathology data and learns to predict precise sTIL% scores for each tile in the tumor bed by using a multiple instance learning regressor that only requires a weak WSI-level label. By requiring only a weak label, we overcome the large annotation efforts required to train currently existing TIL detection methods. We show that WeakSTIL is at least as good as other TIL detection methods when predicting the WSI-level sTIL% score, reaching a coefficient of determination of $0.45\pm0.15$ when compared to scores generated by an expert pathologist, and an AUC of $0.89\pm0.05$ when treating it as the clinically interesting sTIL-high vs sTIL-low classification task. Additionally, we show that the intermediate tile-level predictions of WeakSTIL are highly interpretable, which suggests that WeakSTIL pays attention to latent features related to the number of TILs and the tissue type. In the future, WeakSTIL may be used to provide consistent and interpretable sTIL% predictions to stratify breast cancer patients into targeted therapy arms.

==> WeakSTIL Arxiv (full version) 202109131320/heatmap_figure.tex <==
\begin{figure} [ht]
    \centering
    \includegraphics[width=\textwidth]{fig-heatmap_visualization.pdf}

    \caption{\label{fig:results-visualization} 
    Heatmap visualization of the tile-level sTIL\% scores as predicted by WeakSTIL (HistoSSL-RN18 TILMIL). Left: WeakSTIL receives the tiles of the tumor bed of an H\&E WSI as input, computes an sTIL\% score for each tile, and outputs the mean sTIL\% score of these tiles as WSI-level label score. Right: Close-up of a section of the H\&E WSI. One can see that the model only predicts high sTIL\% scores for TILs that are in stroma, not for TILs that are near tumor cells.
    }
\end{figure}

% \begin{figure} [ht]
%     \centering
%     \begin{subfigure}{0.49\textwidth}
%         \centering
%         \includegraphics[height=0.8\linewidth]{faux-wsi-heatmap.png}
%         \caption[width=\textwidth]{}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.5\textwidth}
%         \begin{subfigure}[b]{0.32\textwidth}
%             \centering
%             \includegraphics[width=\textwidth]{faux-wsi-heatmap.png}
%             \caption[width=\textwidth]{sTIL\%=**}
%         \end{subfigure}
%         \hfill
%         \begin{subfigure}[b]{0.32\textwidth}
%             \centering
%             \includegraphics[width=\textwidth]{faux-wsi-heatmap.png}
%             \caption[width=\textwidth]{sTIL\%=**}
%         \end{subfigure}
%         \hfill
%         \begin{subfigure}[b]{0.32\textwidth}
%             \centering
%             \includegraphics[width=\textwidth]{faux-wsi-heatmap.png}
%             \caption[width=\textwidth]{sTIL\%=**}
%         \end{subfigure}
%     \end{subfigure}
%     %>>>> use \label inside caption to get Fig. number with \ref{}
%     \caption{\label{fig:results-visualization} 
%     (a) a WSI heatmap showing the tile-level sTIL\% score distribution. (b) A tile with many TILs in the tumor bed stroma, correctly receiving a high sTIL\% score. (c) A tile with many TILs in the tumor area of the tumor bed, correctly receiving a low sTIL\% score since it's not in the stroma. (d) A tile with few TILs in the tumor bed stroma, correctly receiving a low sTIL\% score. }
% \end{figure}




% \begin{figure} [ht]
%  %% tabular useful for creating an array of images 
%  \centering
% \begin{subfigure}[b]{0.4\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{faux-wsi-heatmap.png}
%     \caption[width=\textwidth]{}
% \end{subfigure}
% \begin{subfigure}[b]{0.15\textwidth}
%     \begin{subfigure}[b]{\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{faux-wsi-heatmap.png}
%         \caption[width=\textwidth]{sTIL\%=**}
%     \end{subfigure}
%     \begin{subfigure}[b]{\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{faux-wsi-heatmap.png}
%         \caption[width=\textwidth]{sTIL\%=**}
%     \end{subfigure}
%     \begin{subfigure}[b]{\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{faux-wsi-heatmap.png}
%         \caption[width=\textwidth]{sTIL\%=**}
%     \end{subfigure}
% \end{subfigure}
% %>>>> use \label inside caption to get Fig. number with \ref{}
% \caption{\label{fig:results-visualization} 
% (a) a WSI heatmap showing the tile-level sTIL\% score distribution. (b) A tile with many TILs in the tumor bed stroma, correctly receiving a high sTIL\% score. (c) A tile with many TILs in the tumor area of the tumor bed, correctly receiving a low sTIL\% score since it's not in the stroma. (d) A tile with few TILs in the tumor bed stroma, correctly receiving a low sTIL\% score. }
% \end{figure}

==> WeakSTIL Arxiv (full version) 202109131320/hyperparameter_tables.tex <==
\begin{table*}[ht]
\caption{\label{tab:appendix-table-lr-reg-ssl-linear} Results of hyperparameter grid search using HistoSSL-RN18 TILMIL with a single linear layer ($\boldsymbol{w} \in \mathbb{R}^{512}, b \in \mathbb{R}$) for the sTIL\% regression task. Trained for 50 epochs with a batch size of 1, evaluating every epoch, with varying learning rate and regularization, trained on a subsample of 500 tiles. These results are the 5-fold mean and standard deviation on the validation set.}
    \centering
    \begin{tabular}{crrrrrr}
    \toprule
         \multirow{2}{*}{\textbf{Learning rate}}    & \multicolumn{6}{c}{\textbf{Regularization}} \\ 
                            &      $5\times 10^{-3}$ &         $1\times10^{-3}$&   $5\times10^{-4}$ &         $1\times10^{-4}$ &  $5\times10^{-5}$ & $1\times10^{-5}$ \\
    \midrule
         
            $5\times10^{-2}$&   $72.6\pm1.8$ &   $72.1\pm2.4$  & $75.1\pm4.1$& $82.1\pm4.1$  & $83.1\pm5.8$    &   $81.7\pm6.1$\\
            $1\times10^{-2}$       &   $83.8\pm2.9$ &   $85.5\pm3.6$  & $85.2\pm3.4$& $85.2\pm2.4$  & $85.1\pm2.5$    &   $85.5\pm2.2$\\
            $5\times10^{-3}$&   $82.7\pm3.2$ &   $84.0\pm2.6$  & $84.3\pm2.3$& $85.0\pm1.5$  & $84.7\pm1.5$    &   $84.9\pm1.4$\\
            $1\times10^{-3}$       &   $80.5\pm3.4$ &   $80.7\pm3.2$ &  $80.8\pm3.0$& $81.1\pm2.9$  & $81.3\pm2.9$    &   $81.2\pm2.9$\\
            $5\times10^{-4}$&   $79.5\pm3.6$ &   $79.9\pm3.5$ &  $79.9\pm3.5$& $80.1\pm3.4$  & $80.0\pm3.4$    &   $80.0\pm3.4$\\
            $1\times10^{-4}$       &   $76.9\pm4.1$ &   $77.3\pm4.4$ &  $77.3\pm4.5$& $77.3\pm4.6$  & $77.3\pm4.6$    &   $77.3\pm4.6$\\
            $5\times10^{-5}$&   $74.2\pm5.3$ &   $74.5\pm5.4$ &  $74.5\pm5.4$& $74.5\pm5.4$  & $74.5\pm5.4$    &   $74.5\pm5.4$\\
            $1\times10^{-5}$       &   $64.2\pm8.0$ &   $64.0\pm8.0$ &  $64.0\pm8.0$& $63.9\pm8.0$  & $63.9\pm8.0$    &   $63.9\pm8.0$\\ 
    \bottomrule
    \end{tabular}
\end{table*}

\begin{table*}[ht]
\caption{\label{tab:appendix-table-lr-reg-ssl-non-linear} Results of hyperparameter grid search using HistoSSL-RN18 TILMIL with two linear layers ($\boldsymbol{w}_1 \in \mathbb{R}^{512\times128}, b_1 \in \mathbb{R}^{128}$, $\boldsymbol{w}_2 \in \mathbb{R}^{128}, b_2 \in \mathbb{R}$) for the sTIL\% regression task. Trained for 50 epochs with a batch size of 1, evaluating every epoch, with varying learning rate and regularization, trained on a subsample of 500 tiles. These results are the 5-fold mean and standard deviation on the validation set.}
    \centering
    \begin{tabular}{crrrrrr}
    \toprule
         \multirow{2}{*}{\textbf{Learning rate}}    & \multicolumn{6}{c}{\textbf{Regularization}} \\ 
                            &      $5\times 10^{-3}$ &         $1\times10^{-3}$&   $5\times10^{-4}$ &         $1\times10^{-4}$ &  $5\times10^{-5}$ & $1\times10^{-5}$ \\ 
    \midrule
            $5\times10^{-2}$&   $70.4\pm4.1$ &   $67.4\pm3.3$  & $68.2\pm4.1$& $67.0\pm4.1$  & $69.3\pm6.0$    &   $72.3\pm7.8$\\
            $1\times10^{-2}$       &   $79.5\pm2.4$ &   $76.3\pm6.8$  & $71.5\pm7.1$& $79.2\pm5.6$  & $80.9\pm7.4$    &   $69.2\pm3.1$\\
            $5\times10^{-3}$&   $80.4\pm3.1$ &   $84.8\pm3.0$  & $85.6\pm3.5$& $84.0\pm3.3$  & $84.2\pm3.0$    &   $84.0\pm3.4$\\
            $1\times10^{-3}$       &   $80.2\pm3.6$ &   $83.4\pm3.3$ &  $84.0\pm2.9$& $84.3\pm2.2$  & $84.1\pm2.3$    &   $84.2\pm2.3$\\
            $5\times10^{-4}$&   $80.3\pm3.6$ &   $83.0\pm3.5$ &  $83.3\pm3.2$& $83.5\pm2.7$  & $83.5\pm2.6$    &   $83.3\pm2.6$\\
            $1\times10^{-4}$       &   $79.9\pm3.5$ &   $81.1\pm3.1$ &  $81.3\pm3.0$& $81.7\pm2.7$  & $81.8\pm2.7$    &   $81.7\pm2.6$\\
            $5\times10^{-5}$&   $78.9\pm3.6$ &   $79.7\pm3.3$ &  $80.0\pm3.2$& $80.2\pm3.0$  & $80.2\pm3.0$    &   $80.2\pm3.1$\\
            $1\times10^{-5}$       &   $75.1\pm4.9$ &   $75.9\pm4.7$ &  $75.9\pm4.7$& $76.0\pm4.7$  & $76.0\pm4.7$    &   $76.0\pm4.6$\\ 
    \bottomrule    
    \end{tabular}
\end{table*}

\begin{table*}[ht]
\caption{\label{tab:appendix-table-lr-reg-ssl-double-head} Results of hyperparameter grid search using HistoSSL-RN18 TILMIL with two linear layers and a tanh non-linearity after the first layer ($\boldsymbol{w}_1 \in \mathbb{R}^{512\times128}, b_1 \in \mathbb{R}^{128}$, $\boldsymbol{w}_2 \in \mathbb{R}^{128}, b_2 \in \mathbb{R}$) for the sTIL\% regression task. Trained for 50 epochs with a batch size of 1, evaluating every epoch, with varying learning rate and regularization, trained on a subsample of 500 tiles. These results are the 5-fold mean and standard deviation on the validation set.}
    \centering
    \begin{tabular}{crrrrrr}
    \toprule
         \multirow{2}{*}{\textbf{Learning rate}}    & \multicolumn{6}{c}{\textbf{Regularization}} \\ 
                            &      $5\times 10^{-3}$ &         $1\times10^{-3}$&   $5\times10^{-4}$ &         $1\times10^{-4}$ &  $5\times10^{-5}$ & $1\times10^{-5}$ \\
    \midrule
            $5\times10^{-2}$&   $70.8\pm2.7$ &   $69.0\pm2.6$  & $70.9\pm2.0$& $68.5\pm1.4$  & $68.5\pm3.3$    &   $69.0\pm5.6$\\
            $1\times10^{-2}$       &   $73.5\pm1.9$ &   $76.8\pm2.3$  & $76.2\pm2.5$& $84.6\pm4.3$  & $84.6\pm3.2$    &   $83.3\pm3.1$\\
            $5\times10^{-3}$&   $75.0\pm3.6$ &   $85.2\pm4.4$  & $86.3\pm3.8$& $84.7\pm3.6$  & $86.0\pm3.4$    &   $85.6\pm4.0$\\
            $1\times10^{-3}$       &   $80.6\pm3.0$ &   $83.9\pm3.0$ &  $84.4\pm3.2$& $84.3\pm2.9$  & $84.3\pm2.9$    &   $84.4\pm2.6$\\
            $5\times10^{-4}$&   $80.5\pm3.3$ &   $83.3\pm3.6$ &  $83.5\pm3.4$& $83.5\pm2.8$  & $83.5\pm2.6$    &   $83.8\pm2.5$\\
            $1\times10^{-4}$       &   $79.9\pm3.5$ &   $81.1\pm3.1$ &  $81.3\pm3.0$& $81.6\pm2.7$  & $81.6\pm2.7$    &   $81.8\pm2.7$\\
            $5\times10^{-5}$&   $78.9\pm3.6$ &   $79.7\pm3.4$ &  $79.9\pm3.3$& $80.2\pm3.2$  & $80.2\pm3.2$    &   $80.3\pm3.1$\\
            $1\times10^{-5}$       &   $75.1\pm4.9$ &   $75.9\pm4.8$ &  $76.0\pm4.8$& $76.1\pm4.8$  & $76.1\pm4.8$    &   $76.1\pm4.8$\\ 
    \bottomrule       
    \end{tabular}
\end{table*}

\begin{table*}[ht]
\caption{\label{tab:appendix-table-lr-reg-imagenet-linear} Results of hyperparameter grid search using IN-RN18 TILMIL with a single linear layer ($\boldsymbol{w} \in \mathbb{R}^{512}, b \in \mathbb{R}$) for the sTIL\% regression task. Trained for 50 epochs with a batch size of 1, evaluating every epoch, with varying learning rate and regularization, trained on a subsample of 500 tiles. These results are the 5-fold mean and standard deviation on the validation set.}
    \centering
    \begin{tabular}{crrrrrr}
    \toprule
         \multirow{2}{*}{\textbf{Learning rate}}    & \multicolumn{6}{c}{\textbf{Regularization}} \\ 
                            &      $5\times 10^{-3}$ &         $1\times10^{-3}$&   $5\times10^{-4}$ &         $1\times10^{-4}$ &  $5\times10^{-5}$ & $1\times10^{-5}$ \\ 
    \midrule
            $5\times10^{-2}$&   $65.5\pm5.5$ &   $66.1\pm5.0$  & $65.3\pm4.8$& $65.1\pm5.0$  & $62.9\pm5.2$    &   $65.2\pm5.8$\\
            $1\times10^{-2}$       &   $65.7\pm5.1$ &   $65.4\pm5.2$  & $65.5\pm4.7$& $64.2\pm5.6$  & $64.3\pm5.1$    &   $63.7\pm4.9$\\
            $5\times10^{-3}$&   $65.9\pm5.6$ &   $64.5\pm5.5$  & $63.3\pm6.1$& $62.7\pm5.4$  & $62.4\pm5.6$    &   $61.7\pm6.5$\\
            $1\times10^{-3}$       &   $58.0\pm6.8$ &   $59.1\pm6.9$ &  $59.2\pm6.9$& $59.3\pm6.9$  & $59.3\pm6.9$    &   $59.3\pm6.9$\\
            $5\times10^{-4}$&   $53.3\pm5.1$ &   $53.2\pm4.9$ &  $53.2\pm4.8$& $53.2\pm4.9$  & $53.2\pm4.9$    &   $53.1\pm4.9$\\
            $1\times10^{-4}$       &   $51.9\pm4.7$ &   $51.5\pm4.6$ &  $51.4\pm4.6$& $51.4\pm4.6$  & $51.4\pm4.6$    &   $51.4\pm4.6$\\
            $5\times10^{-5}$&   $50.4\pm4.3$ &   $50.4\pm4.4$ &  $50.3\pm4.3$& $50.3\pm4.3$  & $50.3\pm4.3$    &   $50.3\pm4.3$\\
            $1\times10^{-5}$       &   $49.7\pm3.1$ &   $49.7\pm3.1$ &  $49.7\pm3.1$& $49.7\pm3.1$  & $49.7\pm3.1$    &   $49.7\pm3.1$\\ 
    \bottomrule
    \end{tabular}
\end{table*}

==> WeakSTIL Arxiv (full version) 202109131320/roc_figure.tex <==


\begin{figure}[t!]
    \centering
    \begin{tabular}{lc lc}
        & ROC for ImageNet-RN18 TILMIL
        & & ROC for HistoSSL-RN18 TILMIL\\
        \rotatebox[origin=c]{90}{True positive rate} &
        \begin{subfigure}{0.4\textwidth}
            \centering
            \includegraphics[width=.8\textwidth]{fig-roc-Receiver_operating_characteristic_for_ImageNet-RN18_TILMIL_Sat_Jul_31_21-38-52_2021.pdf}
        \end{subfigure} \vspace{0.3ex} &
         &
        \begin{subfigure}{0.4\textwidth}
            \centering
            \includegraphics[width=.8\textwidth]{fig-roc-Receiver_operating_characteristic_for_HistoSSL-RN18_TILMIL_Sat_Jul_31_21-28-03_2021.pdf}
        \end{subfigure} \vspace{0.3ex} \\
        & \subfloat[]{False positive rate} & & \subfloat[]{False positive rate}
    \end{tabular}
    \caption{\label{fig:results-roc} 
    Receiver Operating Characteristic curves for the 5 folds of (a) IN-RN18 and (b) HistoSSL-RN18 TILMIL model when comparing the predicted sTIL\% score to the sTIL\% score binarized at a cut-off of $20\%$.}
\end{figure}


% \begin{figure}[!t]
%  %% tabular useful for creating an array of images  
%     \centering
%     \begin{subfigure}[b]{0.4\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{fig-roc-Receiver_operating_characteristic_for_ImageNet-RN18_TILMIL_Sat_Jul_31_21-38-52_2021.pdf}
%     \caption[width=\textwidth]{}
% \end{subfigure}
% \begin{subfigure}[b]{0.4\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{fig-roc-Receiver_operating_characteristic_for_HistoSSL-RN18_TILMIL_Sat_Jul_31_21-28-03_2021.pdf}
%     \caption[width=\textwidth]{}
% \end{subfigure}
    
% \caption{\label{fig:results-roc} 
% Receiver Operating Characteristic curves for the 5 folds of (a) IN-RN18 and (b) HistoSSL-RN18 TILMIL model when comparing the predicted sTIL\% score to the sTIL\% score binarized at a cut-off of $20\%$.}
% \end{figure}

% % 

==> WeakSTIL Arxiv (full version) 202109131320/scatter_plot.tex <==
\begin{figure}[!t]
    \centering
    \setlength{\tabcolsep}{0pt}% Remove space between tabular columns
    \begin{tabular}{p{1em}ccccc}
        \rotatebox[origin=c]{90}{sTILs true} &
        \begin{subfigure}{0.18\textwidth}
            \centering
            \includegraphics[width=\textwidth]{fig-scatter-0_Scatter_HistoSSL-RN18_TILMIL_Sat_Jul_31_21-28-04_2021_r_0.8115394811198999_p_1.107402188953894e-14_R2_0.47704548117555334.pdf}
        \end{subfigure} \vspace{0.1ex}

        &
        \begin{subfigure}{0.18\textwidth}
            \centering
            \includegraphics[width=\textwidth]{fig-scatter-1_Scatter_HistoSSL-RN18_TILMIL_Sat_Jul_31_21-28-04_2021_r_0.8508516573080451_p_1.0178871848589103e-16_R2_0.27546615117276196.pdf}
        \end{subfigure} \vspace{0.1ex}

        &
        \begin{subfigure}{0.18\textwidth}
            \centering
            \includegraphics[width=\textwidth]{fig-scatter-2_Scatter_HistoSSL-RN18_TILMIL_Sat_Jul_31_21-28-04_2021_r_0.8667838625361268_p_1.4580608103897267e-18_R2_0.6776756911492572.pdf}
            
        \end{subfigure} \vspace{0.1ex}
        &
        \begin{subfigure}{0.18\textwidth}
            \centering
            \includegraphics[width=\textwidth]{fig-scatter-3_Scatter_HistoSSL-RN18_TILMIL_Sat_Jul_31_21-28-04_2021_r_0.715598180859937_p_5.719378132778801e-10_R2_0.29736017341630805.pdf}
            
        \end{subfigure} \vspace{0.1ex}
        &
        \begin{subfigure}{0.18\textwidth}
            \centering
            \includegraphics[width=\textwidth]{fig-scatter-4_Scatter_HistoSSL-RN18_TILMIL_Sat_Jul_31_21-28-04_2021_r_0.8550400153024547_p_1.31839995634314e-17_R2_0.544610204442502.pdf}
        \end{subfigure} \vspace{0.1ex}

        \\
        & \subfloat[$r = 0.81^*$]{sTILs Predicted} & \subfloat[$r = 0.85^*$]{sTILs Predicted} & \subfloat[$r = 0.87^*$]{sTILs Predicted} & \subfloat[$r = 0.72^*$]{sTILs Predicted} & \subfloat[$r = 0.86^*$]{sTILs Predicted}
    \end{tabular}
    \caption{\label{fig:results-scatter} Scatter plots comparing the predicted WSI-level sTIL\% score to the pathologist-annotated sTIL\% score for the HistoSSL-RN18 TILMIL model for each fold. The caption states the correlation between the predicted sTIL\% score and the actual sTIL\% score. (a) Fold 1: $R^2=0.48$, (b) Fold 2: $R^2=0.28$, (c) Fold 3: $R^2=0.68$, (d) Fold 4: $R^2=0.30$, (e) Fold 5: $R^2=0.54$. $^{*}: p<0.001$}
\end{figure}


% \begin{figure}[t]

% %% tabular useful for creating an array of images 
% \centering
% \begin{subfigure}[b]{0.18\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{fig-scatter-0_Scatter_HistoSSL-RN18_TILMIL_Sat_Jul_31_21-28-04_2021_r_0.8115394811198999_p_1.107402188953894e-14_R2_0.47704548117555334.pdf}
%     \caption[width=\textwidth]{$r = 0.81^*$}
% \end{subfigure}
% \begin{subfigure}[b]{0.18\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{fig-scatter-1_Scatter_HistoSSL-RN18_TILMIL_Sat_Jul_31_21-28-04_2021_r_0.8508516573080451_p_1.0178871848589103e-16_R2_0.27546615117276196.pdf}
%     \caption[width=\textwidth]{$r = 0.85^*$}
% \end{subfigure}
% \begin{subfigure}[b]{0.18\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{fig-scatter-2_Scatter_HistoSSL-RN18_TILMIL_Sat_Jul_31_21-28-04_2021_r_0.8667838625361268_p_1.4580608103897267e-18_R2_0.6776756911492572.pdf}
%     \caption[width=\textwidth]{$r = 0.87^*$}
% \end{subfigure}
% \begin{subfigure}[b]{0.18\textwidth}
%     \centering
%     \includegraphics[width=\textwidth     ]{fig-scatter-3_Scatter_HistoSSL-RN18_TILMIL_Sat_Jul_31_21-28-04_2021_r_0.715598180859937_p_5.719378132778801e-10_R2_0.29736017341630805.pdf}
%     \caption[width=\textwidth]{$r = 0.72^*$}
% \end{subfigure}
% \begin{subfigure}[b]{0.18\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{fig-scatter-4_Scatter_HistoSSL-RN18_TILMIL_Sat_Jul_31_21-28-04_2021_r_0.8550400153024547_p_1.31839995634314e-17_R2_0.544610204442502.pdf}
%     \caption[width=\textwidth]{$r = 0.86^*$}
% \end{subfigure}
% \caption[example] 
% %>>>> use \label inside caption to get Fig. number with \ref{}
% {\label{fig:results-scatter} 
% Scatter plots comparing the predicted WSI-level sTIL\% score to the pathologist-annotated sTIL\% score for the HistoSSL-RN18 TILMIL model for each fold. The caption states the correlation between the predicted sTIL\% score and the actual sTIL\% score. (a) $R^2=0.48$, (b) Fold 1: $R^2=0.28$, (c) Fold 2: $R^2=0.68$, (d) Fold 3: $R^2=0.30$, (e) Fold 4: $R^2=0.54$. $^{*}: p<0.001$}
% \end{figure} 
